Active Learning based on Data Uncertainty and Model Sensitivity

Robots can rapidly acquire new skills from demonstrations. However, during generalisation of skills or transitioning across fundamentally different skills, it is unclear whether the robot has the necessary knowledge to perform the task. Failing to detect missing information often leads to abrupt movements or to collisions with the environment. Active learning can quantify the uncertainty of performing the task and, in general, locate regions of missing information. We introduce a novel algorithm for active learning and demonstrate its utility for generating smooth trajectories. Our approach is based on deep generative models and metric learning in latent spaces. It relies on the Jacobian of the likelihood to detect non-smooth transitions in the latent space, i.e., transitions that lead to abrupt changes in the movement of the robot. When non-smooth transitions are detected, our algorithm asks for an additional demonstration from that specific region. The newly acquired knowledge modifies the data manifold and allows for learning a latent representation for generating smooth movements. We demonstrate the efficacy of our approach on generalising elementary skills, transitioning across different skills, and implicitly avoiding collisions with the environment. For our experiments, we use a simulated pendulum where we observe its motion from images and a 7-DoF anthropomorphic arm.

==> sections/related_work2.tex <==
%!TEX root = ../active_learning.tex
\section{Related work} % (fold)
\label{sec:related_work}

% section related_work (end)

There are three types of active learning in terms of the scenarios \cite{settles2010active}. In membership queries synthesis scenario (e.g., \cite{angluin1988queries, king2009automation}), instead of sampling from natural distributions, the learner probably requests annotations for any unlabelled instance in the input space. Another scenario is stream-based selective sampling (e.g., \cite{atlas1990training}). The assumption is that obtaining unlabelled instances is cheap. A sample can be generated from the distribution, and then the learner decides to request or discard the corresponding label. The third scenario is pool-based sampling (e.g., \cite{lewis1994sequential, Gal2017Active}). In some real-world learning problems, large unlabelled data can be collected. In the pool-based sampling scenario, the assumption is that a large number of unlabelled data is provided and the labeled data set size is small. Labels are requested from the pool of the unlabelled data. In our illustrative experiment in Section~\ref{toy_experiment}, pool-based sampling is used. Although it is an unsupervised learning task and does not require labels, we select most useful data from the pool to evaluate our method. In Section~\ref{pendulum_experiment} and \ref{robot_experiment}, it is expensive to obtain the unlabelled data in these robot scenarios, so the stream-based selective sampling is used. In our method, the trajectory samples are obtained using geodesics.
% reader: active learning servey

Current algorithms of active learning mainly contain uncertainty sampling \cite{tong2001support}, query by committee \cite{seung1992query} and expected error reduction \cite{roy2001toward}. 
Existing work on uncertainty sampling commonly uses kernel-based methods. 
For instance, ``margin-based uncertainty'' for support vector machines is applicable to low-dimensional data \cite{joshi2009multi}.  
\cite{li2013adaptive} combined RBF kernels with information density and the uncertainty of Gaussian processes. 
\cite{zhu2003combining} acquired data using a Gaussian random field model and employed an RBF kernel over raw image data.
Following \cite{pmlr_v51_que16}, we used RBF networks to model data uncertainty.
% In contrast, most of the deep learning-based methods are not capable to model such uncertainty. 
% reader: Learning how to Active Learn: A Deep Reinforcement Learning Approach--related work
% reader: https://www.cs.cmu.edu/~tom/10701_sp11/recitations/Recitation_13.pdf

%Thus, we take the advantage of the kernel based approaches and adapt it to the deep learning
%However, \cite{pmlr_v51_que16} introduced an approach to approximate uncertainty with latent variable models by adding an RBF network to the generative model. We follow this line to use the RBF for 

% Except of data uncertainty, detection of model defects (for instance, the model uncertainty) is also used for active learning. 
Recent work \cite{Gal2017Active} introduced Bayesian deep learning for the active learning framework for image classification. Our method is an alternative for model defect detection by measuring model sensitivity. 


In robotics, active learning is widely used, especially, along with reinforcement learning. Active learning is used for agent querying the actions \cite{atlas1990training, cohn1996active} or exploring the actions \cite{salganicoff1996active, morales2004active}. Active learning and reactive control are used for robot grasping \cite{kroemer2010combining}. In robot motion, \cite{maeda2017active} used the uncertainty of Gaussian processes to query new demonstrations. In the latter work however, the user still has to manually choose the trigger.
% reader: Skill Learning by Autonomous Robotic Playing using Active Learning and Creativity

%In robotics, active learning is widely used along with reinforcement learning. \cite{chernova2009interactive} introduce Confidence-Based Autonomy for policy learning from demonstrations by actively requesting new demonstrations. In robot motion, \cite{maeda2017active} used the uncertainty of Gaussian processes to query new demonstrations. In the latter work however, the user still has to manually choose the trigger. Finally, \cite{silver2012active} introduced novelty and uncertainty reduction for navigation.



%These methods are on low dimension. Our method can deal with high-dimensional data, e.g., pendulum image.


